Portfolio Risk Bounds without Cross-Asset Return Covariances: Distributional Fields from Language-Model Representations

Portfolio risk assessment ordinarily relies on reliable estimates of cross-asset return covariances, which are difficult to obtain in short, high-dimensional panels. We show that firm-level distribution-valued characteristics can instead provide one-sided certificates of portfolio risk. Under maintained links from characteristics to systematic exposures and from exposures to returns, multi-firm Wasserstein-2 dispersion yields a sharp upper bound on systematic portfolio variance and a corresponding bound for standardized returns. A weighted pairwise relaxation produces an objective that is convex under a checkable condition and requires marginal volatility scales but no cross-asset return covariances. With zero firm-specific slack, the common-map scale changes the certified variance reduction but not the normalized allocation, which depends only on observed information geometry. In a 100-firm panel from 2018-2022, only 0.09%-0.46% of portfolios across four prespecified capped reference populations have in-sample variance no greater than an allocation constructed from Qwen3-Embedding-8B news representations; the corresponding share for equal risk weighting is 28.3%-34.7%. The lower in-sample variance ranking relative to equal risk also appears across the reported frozen language-model representations. The framework therefore converts distribution-valued firm information into a coherent risk bound and an implementable allocation rule constructed without cross-asset return covariances.

==> chapters/statements.tex <==
% Required by the EJF editorial office (11 Sep 2026): disclosure, funding, and
% a data availability statement, all placed between the conclusions and the
% references. \ppanonymous is defined only by the anonymous submission target,
% where the repository identifiers would name the authors.
\section*{Disclosure of interest}

The authors report there are no relevant financial or non-financial competing
interests to declare.

\section*{Funding}

No funding was received.

\section*{Data availability statement}

\ifdefined\ppanonymous
The code that produces every result in this article is publicly archived under
a persistent identifier, and the redistributable derived data are openly
available in a public repository from which the reported artifacts reproduce
exactly. Both identifiers name the authors and are therefore withheld from this
anonymised manuscript; they are recorded in the submission system and will
appear in the version of record.
\else
The code that produces every result in this article is openly available at
\url{https://doi.org/10.5281/zenodo.22689255}, and is mirrored at
\url{https://github.com/marcusinthesky/PricingPerspective}. The redistributable
derived data are openly available at
\url{https://huggingface.co/collections/marcusinthesky/pricingperspective}, and
the reported artifacts reproduce exactly from that public store through the
content hashes recorded in the accompanying code.
\fi

\section*{Declaration of generative AI use}

Generative AI assistants were used in preparing this article --- Codex
0.146.0 and Claude Code 2.1.223 --- for ideation, code refactoring, and
editorial review. No text, result, or reference entered the manuscript without
author verification. The authors confirm that the content is original, have
checked each tool's terms of use, and take full responsibility for the
integrity of the whole article, including the accuracy of all references.
\ifdefined\ppanonymous
The tool versions are pinned in the replication code, whose identifiers are
withheld from this anonymised manuscript.
\else
The specific tools and versions are published alongside our replication code.
\fi

